A combined finite element-finite volume framework for phase-field fracture

Numerical simulations of brittle fracture using phase-field approaches often employ a discrete approximation framework that applies the same order of interpolation for the displacement and phase-field variables. Most common is to use linear finite elements to discretize the linear momentum and phase-field equations. However the use of $P_1$ Lagrange shape functions to model the phase-field is not optimal, since the latter develops cusps for fully developed cracks that in turn occur at locations correspoding to Gauss points of the associated FE model for the mechanics. Such feature is challenging to reproduce accurately with low order elements, and consequently element sizes must be made very small relative to the phase-field regularization parameter in order to achieve convergence of results with respect to the mesh. In this paper, we combine the standard $P_1$ FE discretization of stress equilibrium with a cell-centered finite volume approximation of the phase-field evolution equation based on the two-point flux approximation that is constructed on the same simplex mesh. Compared to a pure FE formulation utilizing linear elements, the proposed framework results in looser restrictions on mesh refinement with respect to the phase-field length scale. Furthermore, initialization of the history field is straightforward and accomplished through a local procedure. The ability to employ a coarser mesh relative to the traditional implementation is shown for several numerical examples, demonstrating savings in computational cost on the order of 50 to 80 percent for the studied cases.

==> implementation-aspects.tex <==
\section{Implementation aspects}
To compare the performance of our proposed mixed FE/FV scheme with traditional discretizations involving equal order FE basis functions for both $\mathbf{u}$ and $\phi$, we implement both formulations within the software framework BROOMStyx, a general multiphysics simulator developed by the first author that allows for combination of different discretization schemes with minimal overhead. The pure FE discretization has been coded to use P1 elements, which enables us to run both formulations with the exactly the same meshes. Implementations for both schemes are optimized by pre-calculating quantities such as gradient matrices that do not vary with time at each evaluation point. Note that the incurred memory footprint of this is larger for the pure FE scheme in the phase-field subsystem, which requires storage of both a 2-by-3 gradient matrix and 3-by-3 mass matrix (see implementation details from Sargado et al., 2018). In contrast, the mixed FE/FV scheme only needs to store transmissibility coefficients, i.e. a single scalar value per local cell edge. The code is designed to run in parallel on shared memory architectures by means of OpenMP directives, and dense matrix operations are carried out using BLAS and LAPACK routines provided by the Intel Math Kernel Library (MKL). Likewise, shared memory-parallel solution of sparse linear systems is obtained via MKL version of the direct solver PARDISO. 
No adaptive remeshing is performed during the course of simulations, hence the initial sparsity profiles of global coefficient matrix do not change. This property is exploited the same way as in Sargado et al., 2018 to speed up the solution of linear systems, specifically by performing symbolic factorization only at the beginning iteration of a substep, and thereafter proceeding directly to the numerical factorization phase of the solver in subsequent iterations. Additionally since both schemes produce symmetric global coefficient matrices, only the upper triangular portion of said matrices are actually assembled and manipulated by the linear solver which cuts down further the time for each iteration.
